A Causal Intervention Scheme for Semantic Segmentation of Quasi-periodic Cardiovascular Signals

Precise segmentation is a vital first step to analyze semantic information of cardiac cycle and capture anomaly with cardiovascular signals. However, in the field of deep semantic segmentation, inference is often unilaterally confounded by the individual attribute of data. Towards cardiovascular signals, quasi-periodicity is the essential characteristic to be learned, regarded as the synthesize of the attributes of morphology (Am) and rhythm (Ar). Our key insight is to suppress the over-dependence on Am or Ar while the generation process of deep representations. To address this issue, we establish a structural causal model as the foundation to customize the intervention approaches on Am and Ar, respectively. In this paper, we propose contrastive causal intervention (CCI) to form a novel training paradigm under a frame-level contrastive framework. The intervention can eliminate the implicit statistical bias brought by the single attribute and lead to more objective representations. We conduct comprehensive experiments with the controlled condition for QRS location and heart sound segmentation. The final results indicate that our approach can evidently improve the performance by up to 0.41% for QRS location and 2.73% for heart sound segmentation. The efficiency of the proposed method is generalized to multiple databases and noisy signals.

==> backup.tex <==
\appendices

\begin{table*}[!ht]
\centering
\label{tab:1}
\caption{Comparison results of QRS location using the same MBCNN as the backbone model, where the best $F_1$ results are marked in bold. The better results are \textbf{bold-faced}.
}
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{1.2mm}
\begin{tabular}{llllllllll}
\hline
Database      & Method & TP & FP & FN & & Se & PPR & ER & F1    \\
\hline\hline
CPSC2019-TEST & MBCNN & 42772$\pm$83 & 394$\pm$97 & 526$\pm$83 & & 98.79$\pm$0.19 
              & 99.09$\pm$0.22 & 2.10$\pm$0.24 & 98.94$\pm$0.12 \\

              & MBCNN+CCI ($A_m$) & 43002$\pm$22 & 299$\pm$35 & 296$\pm$22 & & \textbf{99.32$\pm$0.05} & 99.31$\pm$0.08 & 1.36$\pm$0.06 & 99.31$\pm$0.03 \\
              
              & MBCNN+CCI ($A_r$) & 42988$\pm$16 & 274$\pm$28 & 310$\pm$16 & & 99.28$\pm$0.04 & 99.37$\pm$0.06 & 1.34$\pm$0.08 & 99.32$\pm$0.04 \\
              
              & MBCNN+CCI ($A_m$ \& $A_r$) & 42976$\pm$15 & 239$\pm$12 & 322$\pm$15 & & 99.26$\pm$0.03  & \textbf{99.45$\pm$0.03} & \textbf{1.29$\pm$0.02} & \textbf{99.35$\pm$0.009} \\
\cline{1-10}
MITDB         & MBCNN     & 217108$\pm$288 & 1217$\pm$271 & 1760$\pm$288 & & 99.20$\pm$0.13 & 99.44$\pm$0.12 & 1.35$\pm$0.10 & 99.32$\pm$0.05 \\

              & MBCNN+CCI ($A_m$) & 217478$\pm$160 & 1106$\pm$157 & 1390$\pm$160 & & 99.37$\pm$0.07 & 99.49$\pm$0.07 & 1.13$\pm$0.06 & 99.43$\pm$0.03 \\
              
              & MBCNN+CCI ($A_r$) & 217572$\pm$75 & 1101$\pm$51 & 1296$\pm$75 & & \textbf{99.41$\pm$0.03} & 99.50$\pm$0.02 & 1.09$\pm$0.02 & 99.45$\pm$0.01 \\
              
              & MBCNN+CCI ($A_m$ \& $A_r$) & 217509$\pm$97 & 961$\pm$71 & 1359$\pm$97 & & 99.38$\pm$0.04 & \textbf{99.56$\pm$0.03} & \textbf{1.06$\pm$0.06} & \textbf{99.47$\pm$0.03} \\
\cline{1-10}
INCART        & MBCNN    & 2090962$\pm$1993 & 18389$\pm$4484 & 13726$\pm$1993 &                          &99.35$\pm$0.09 & 99.13$\pm$0.21 & 1.51$\pm$0.13 & 99.24$\pm$0.06 \\
              
              & MBCNN+CCI ($A_m$) & 2093182$\pm$1014 & 15183$\pm$2010 & 11506$\pm$1014 & & 99.45$\pm$0.05 & 99.28$\pm$0.09 & 1.26$\pm$0.06 & 99.37$\pm$0.03 \\
              
              & MBCNN+CCI ($A_r$) & 2093728$\pm$731 & 16305$\pm$1798 & 10960$\pm$731 & & \textbf{99.48$\pm$0.03} & 99.23$\pm$0.08 & 1.29$\pm$0.07 & 99.35$\pm$0.03 \\
              
              & MBCNN+CCI ($A_m$ \& $A_r$) & 2093131$\pm$861 & 14296$\pm$754 & 11557$\pm$861 & & 99.45$\pm$0.04 & \textbf{99.32$\pm$0.04} & \textbf{1.22$\pm$0.03} & \textbf{99.39$\pm$0.02} \\
\cline{1-10}
QT            & MBCNN     & 141027$\pm$54 & 138$\pm$37 & 93$\pm$54 & & 
              99.93$\pm$0.04 & 99.90$\pm$0.03 & 0.16$\pm$0.03 & 99.92$\pm$0.02 \\
              
              & MBCNN+CCI ($A_m$) & 141077$\pm$22 & 101$\pm$20 & 43$\pm$22 & & 99.97$\pm$0.02 & 99.93$\pm$0.01 & 0.10$\pm$0.02 & 99.95$\pm$0.01 \\
              
              & MBCNN+CCI ($A_r$) & 141089$\pm$6 & 114$\pm$23 & 31$\pm$6 & & \textbf{99.98$\pm$0.004} & 99.92$\pm$0.02 & 0.10$\pm$0.02 & \textbf{99.95$\pm$0.009} \\
              
              & MBCNN+CCI ($A_m$ \& $A_r$) & 141056$\pm$36 & 77$\pm$17 & 64$\pm$36 & & 99.95$\pm$0.03 & \textbf{99.95$\pm$0.01} & \textbf{0.10$\pm$0.02} & 99.95$\pm$0.01 \\
\cline{1-10}  
\end{tabular}
\end{table*}

\begin{table}[h]
\centering
\label{tab:1}
\caption{Comparison results of QRS location using the same MBCNN as the backbone Encoder. The better results are \textbf{bold-faced}.
}

\begin{tabular}{lllll}
\hline

Database      & Method & $Se$ & $P_+$ & $F_1$    \\
\hline\hline
CPSC2019      & MBCNN & 98.79$\pm$0.19 
              & 99.09$\pm$0.22 & 98.94$\pm$0.12 \\

              & MBCNN+CCI ($A_m$) & \textbf{99.32$\pm$0.05} & 99.31$\pm$0.08 & 99.31$\pm$0.03 \\
              
              & MBCNN+CCI ($A_r$) & 99.28$\pm$0.04 & 99.37$\pm$0.06 & 99.32$\pm$0.04 \\
              
              & MBCNN+CCI ($A_m$ \& $A_r$) & 99.26$\pm$0.03  & \textbf{99.45$\pm$0.03} & \textbf{99.35$\pm$0.009} \\
\cline{1-5}
MITDB         & MBCNN     & 99.20$\pm$0.13 & 99.44$\pm$0.12 & 99.32$\pm$0.05 \\

              & MBCNN+CCI ($A_m$) & 99.37$\pm$0.07 & 99.49$\pm$0.07 & 99.43$\pm$0.03 \\
              
              & MBCNN+CCI ($A_r$) & \textbf{99.41$\pm$0.03} & 99.50$\pm$0.02 & 99.45$\pm$0.01 \\
              
              & MBCNN+CCI ($A_m$ \& $A_r$) & 99.38$\pm$0.04 & \textbf{99.56$\pm$0.03} & \textbf{99.47$\pm$0.03} \\
\cline{1-5}
INCART        & MBCNN     &99.35$\pm$0.09 & 99.13$\pm$0.21 & 99.24$\pm$0.06 \\
              
              & MBCNN+CCI ($A_m$) & 99.45$\pm$0.05 & 99.28$\pm$0.09 & 99.37$\pm$0.03 \\
              
              & MBCNN+CCI ($A_r$) & \textbf{99.48$\pm$0.03} & 99.23$\pm$0.08 & 99.35$\pm$0.03 \\
              
              & MBCNN+CCI ($A_m$ \& $A_r$) & 99.45$\pm$0.04 & \textbf{99.32$\pm$0.04} & \textbf{99.39$\pm$0.02} \\
\cline{1-5}
QT            & MBCNN     &99.93$\pm$0.04 & 99.90$\pm$0.03 & 99.92$\pm$0.02 \\
              
              & MBCNN+CCI ($A_m$) & 99.97$\pm$0.02 & 99.93$\pm$0.01 & 99.95$\pm$0.01 \\
              
              & MBCNN+CCI ($A_r$) & \textbf{99.98$\pm$0.004} & 99.92$\pm$0.02 & \textbf{99.95$\pm$0.009} \\
              
              & MBCNN+CCI ($A_m$ \& $A_r$) & 99.95$\pm$0.03 & \textbf{99.95$\pm$0.01} & 99.95$\pm$0.01 \\
\cline{1-5}  
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Comparison results of $F_1$ (\%) for QRS location with and without data augmentation of intervened training data. MBCNN is used as the basic Encoder. The better results are \textbf{bold-faced}.}
\label{tab:2}
\begin{tabular}{lllll}
\hline

\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{1.2mm}

Database      & Method & Se & PPR & F1    \\
\hline\hline
CPSC2019-TEST & MBCNN &  98.79 & \textbf{99.09} & 98.94 \\
              & MBCNN+Aug & \textbf{98.81} & 99.07 & \textbf{98.94} \\

\cline{1-5}
MITDB         & MBCNN     & \textbf{99.20} & \textbf{99.44} & \textbf{99.32} \\
              
              & MBCNN+Aug & 99.05 & 99.40 & 99.22 \\

\cline{1-5}
INCART        & MBCNN & \textbf{99.35} & 99.13 & 99.24 \\
              
              & MBCNN+Aug & 99.09 & \textbf{99.47} & \textbf{99.28} \\
              
\cline{1-5}
QT            & MBCNN & \textbf{99.93} & \textbf{99.90} & \textbf{99.92} \\
              
              & MBCNN+Aug & 99.92 & 99.87 & 99.89 \\
\cline{1-5}
    \end{tabular}
\end{table}

\begin{table}[h]
  \centering
  \label{tab:3}
  \caption{Ablation results (\%) for heart sound segmentation with MBCNN as the backbone Encoder. The results are average of five sub models under 5-fold cross validation and the better results are \textbf{bold-faced}.}
  \renewcommand{\arraystretch}{1.25}
  \setlength{\tabcolsep}{1.8mm}
  \begin{tabular}{ccccc}
    \hline
    Database & Method & $Se$ & $P_+$ & $F_1$ \\
    \hline\hline
    \multirow{3}{*}{Training-a} & MBCNN & 95.76$\pm$0.13 & 94.39$\pm$0.30 & 95.07$\pm$0.20 \\
    
    & MBCNN+CCI ($A_m$) & \textbf{96.24$\pm$0.20} & 95.71$\pm$0.18 & 95.97$\pm$0.16 \\
    
    & MBCNN+CCI ($A_r$) & 95.92$\pm$0.20 & 95.59$\pm$0.34 & 95.76$\pm$0.21 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & 96.10$\pm$0.05 & \textbf{95.96$\pm$0.16} & \textbf{96.03$\pm$0.06} \\
    
    \cline{1-5}
    
    \multirow{3}{*}{Training-b} & MBCNN & 87.94$\pm$0.21 & 88.44$\pm$0.90 & 88.19$\pm$0.47 \\
    
    & MBCNN+CCI ($A_m$) & \textbf{89.26$\pm$0.21} & 90.19$\pm$0.20 & 89.72$\pm$0.07 \\
    
    & MBCNN+CCI ($A_r$) & 88.52$\pm$0.42 & 89.96$\pm$0.73 & 89.23$\pm$0.29 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & 89.17$\pm$0.31 & \textbf{90.87$\pm$0.58} & \textbf{90.01$\pm$0.15} \\
    
    \cline{1-5}
    
    \multirow{3}{*}{Training-c} & MBCNN & 89.50$\pm$0.74 & 87.47$\pm$1.13 & 88.47$\pm$0.93 \\
    
    & MBCNN+CCI ($A_m$) & 90.34$\pm$1.10 & 89.51$\pm$0.32 & 89.92$\pm$0.50 \\
    
    & MBCNN+CCI ($A_r$) & 90.06$\pm$0.57 & 89.51$\pm$1.05 & 89.78$\pm$0.72 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & \textbf{90.79$\pm$0.57} & \textbf{90.33$\pm$0.54} & \textbf{90.56$\pm$0.33} \\
    
    \cline{1-5}
    
    \multirow{3}{*}{Training-d} & MBCNN & 95.50$\pm$0.12 & 93.47$\pm$0.39 & 94.47$\pm$0.20 \\
    
    & MBCNN+CCI ($A_m$) & 95.82$\pm$0.39 & 94.06$\pm$0.58 & 94.93$\pm$0.39 \\
    
    & MBCNN+CCI ($A_r$) & 95.69$\pm$0.31 & 94.21$\pm$0.31 & 94.94$\pm$0.30 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & \textbf{95.82$\pm$0.28} & \textbf{94.40$\pm$0.44} & \textbf{95.10$\pm$0.23} \\
    
    \cline{1-5}
    
    \multirow{3}{*}{Training-e} & MBCNN & 89.97$\pm$0.86 & 93.29$\pm$0.57 & 91.60$\pm$0.69 \\
    
    & MBCNN+CCI ($A_m$) & \textbf{91.55$\pm$0.68} & 94.76$\pm$0.49 & 93.12$\pm$0.57 \\
    
    & MBCNN+CCI ($A_r$) & 91.31$\pm$0.48 & 94.82$\pm$0.61 & 93.03$\pm$0.54 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & 91.39$\pm$0.86 & \textbf{95.40$\pm$0.32} & \textbf{93.35$\pm$0.56} \\
    
    \cline{1-5}
    
    \multirow{3}{*}{Training-f} & MBCNN & 84.90$\pm$0.67 & 83.78$\pm$0.85 & 84.33$\pm$0.71 \\
    
    & MBCNN+CCI ($A_m$) & 84.13$\pm$2.73 & 85.74$\pm$2.04 & 84.93$\pm$2.34 \\
    
    & MBCNN+CCI ($A_r$) & 85.38$\pm$0.96 & 87.40$\pm$1.15 & 86.38$\pm$1.01 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & \textbf{85.58$\pm$1.37} & \textbf{88.58$\pm$1.11} & \textbf{87.06$\pm$1.22} \\
    
    \cline{1-5}
    
    \multirow{3}{*}{Test-b} & 87.82$\pm$0.42 & 87.84$\pm$0.83 & 87.83$\pm$0.50 \\
    
    & MBCNN+CCI ($A_m$) & \textbf{89.48$\pm$0.32} & 90.32$\pm$0.50 & \textbf{89.90$\pm$0.27} \\
    
    & MBCNN+CCI ($A_r$) & 88.76$\pm$0.31 & 90.05$\pm$0.81 & 89.40$\pm$0.41 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & 89.28$\pm$0.35 & \textbf{90.33$\pm$0.53} & 89.80$\pm$0.19 \\
    
    \cline{1-5}
    
    \multirow{3}{*}{Test-c} & MBCNN & 94.76$\pm$0.40 & 92.90$\pm$0.56 & 93.82$\pm$0.32 \\
    
    & MBCNN+CCI ($A_m$) & \textbf{95.24$\pm$0.30} & 93.72$\pm$0.36 & 94.47$\pm$0.30 \\
    
    & MBCNN+CCI ($A_r$) & 95.09$\pm$0.43 & 93.74$\pm$0.60 & 94.41$\pm$0.37 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & 95.18$\pm$0.25 & \textbf{94.19$\pm$0.75} & \textbf{94.68$\pm$0.42} \\
    
    \cline{1-5}
    
    \multirow{3}{*}{Test-d} & 96.25$\pm$0.66 & 96.90$\pm$0.21 & 96.57$\pm$0.39  \\
    
    & MBCNN+CCI ($A_m$) & 96.73$\pm$0.45 & 96.57$\pm$0.78 & 96.65$\pm$0.25 \\
    
    & MBCNN+CCI ($A_r$) & 96.73$\pm$0.47 & 97.08$\pm$0.77 & 96.91$\pm$0.47 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & \textbf{96.86$\pm$0.59} & \textbf{97.73$\pm$0.39} & \textbf{97.29$\pm$0.41} \\
    
    \cline{1-5}
    
    \multirow{3}{*}{Test-e} & MBCNN & 95.15$\pm$0.34 & 96.73$\pm$0.19 & 95.93$\pm$0.25  \\
    
    & MBCNN+CCI ($A_m$) & \textbf{95.79$\pm$0.35} & 97.74$\pm$0.29 & 96.76$\pm$0.30 \\
    
    & MBCNN+CCI ($A_r$) & 95.73$\pm$0.26 & 97.56$\pm$0.26 & 96.64$\pm$0.22 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & 95.77$\pm$0.23 & \textbf{97.83$\pm$0.23} & \textbf{96.79$\pm$0.21} \\
    
    \cline{1-5}
    
    \multirow{3}{*}{Test-g} & MBCNN & 89.66$\pm$0.39 & 88.93$\pm$0.57 & 89.29$\pm$0.34  \\
    
    & MBCNN+CCI ($A_m$) & \textbf{90.11$\pm$0.46} & 90.71$\pm$0.33 & 90.41$\pm$0.38 \\
    
    & MBCNN+CCI ($A_r$) & 89.51$\pm$0.35 & 90.26$\pm$0.75 & 89.88$\pm$0.34 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & 89.92$\pm$0.52 & \textbf{91.30$\pm$0.70} & \textbf{90.60$\pm$0.54} \\
    
    \cline{1-5}
    
    \multirow{3}{*}{Test-i} & MBCNN & 92.29$\pm$0.64 & 90.14$\pm$0.56 & 92.17$\pm$0.51  \\
    
    & MBCNN+CCI ($A_m$) & 94.15$\pm$0.34 & 91.54$\pm$0.65 & 92.82$\pm$0.43 \\
    
    & MBCNN+CCI ($A_r$) & 93.41$\pm$0.66 & 91.66$\pm$0.81 & 92.53$\pm$0.70 \\
    
    & MBCNN+CCI ($A_m$ \& $A_r$) & \textbf{94.36$\pm$0.41} & \textbf{92.36$\pm$0.27} & \textbf{93.35$\pm$0.22} \\
    
    \cline{1-5}
    
    \hline
  \end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{The $F_1$ results of common networks used as Encoders with and without CCI for heart sound segmentation on Training-a\textasciitilde f.
Training-$*$ is abbreviated to T$*$ for convenience.
The better results are \textbf{bold-faced}.}
\label{tab:4}
\begin{tabular}{ccccccc}
\hline

\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{1.2mm}

Database      & Ta & Tb & Tc & Td & Te & Tf \\
\hline\hline
DenseNet      & 94.85 & 87.89 & 87.09 & 94.24 & 91.91 & 84.84 \\
DenseNet+CCI  & \textbf{95.96} & \textbf{90.06} & \textbf{90.98} & \textbf{94.93} & \textbf{93.23} & \textbf{86.30} \\

\cline{1-7}
TCN           & 95.76 & 89.22 & 88.12 & 92.90 & 90.95 & \textbf{80.03} \\
TCN+CCI       & \textbf{96.06} & \textbf{90.38} & \textbf{90.19} & \textbf{94.55} & \textbf{92.71} & 79.06 \\

\cline{1-7}
SE-TCN         & 95.78 & 90.02 & 89.92 & 95.14 & 92.16 & 84.40 \\
SE-TCN+CCI     & \textbf{96.29} & \textbf{90.60} & \textbf{90.25} & \textbf{95.36} & \textbf{93.18} & \textbf{85.97} \\
              
\cline{1-7}
\end{tabular}
\end{table}

\section{Training Details for QRS Location and Heart Sound Segmentation}
\label{appendix_a}
\begin{table*}[!h]
\label{tab:6}
    \centering
    \caption{ The network architecture of MBCNN for QRS location. The example for the illustration of a convolution layer is described as Conv1D (kernel size, output channels, dilation rate, activated function). }
    \begin{tabular}{ccc}                                                              \\ \hline
    \multicolumn{3}{c}{Input: 2500*1 ECG episode}                                             \\ \hline \hline
    \multicolumn{3}{c}{Encoder}                                                       \\ \hline \hline
    Branch I                  & Branch II                 & Branch III                \\ \hline
    Conv1D (11, 16, 1, 'Relu') & Conv1D (11, 16, 2, 'Relu') & Conv1D (11, 16, 4, 'Relu') \\
    Conv1D (7, 32, 1, 'Relu')  & Conv1D (7, 32, 2, 'Relu')  & Conv1D (7, 32, 4, 'Relu')  \\
    Conv1D (7, 32, 1, 'Relu')  & Conv1D (7, 32, 4, 'Relu')  & Conv1D (7, 32, 8, 'Relu')  \\ \hline
    \multicolumn{3}{c}{Instance Normalization, MaxPool1D(2)}                          \\ \hline
    Conv1D (5, 64, 1, 'Relu')  & Conv1D (5, 64, 8, 'Relu')  & Conv1D (5, 64, 16, 'Relu') \\
    Conv1D (5, 64, 1, 'Relu')  & Conv1D (5, 64, 8, 'Relu')  & Conv1D (5, 64, 32, 'Relu') \\
    Conv1D (5, 64, 1, 'Relu')  & Conv1D (5, 64, 8, 'Relu')  & Conv1D (5, 64, 64, 'Relu') \\ \hline
    \multicolumn{3}{c}{Instance Normalization, MaxPool1D(2)}                          \\ \hline
    Feat I                    & Feat II                   & Feat III                  \\ \hline
    \multicolumn{3}{c}{Concatenate (Feat I, Feat II, Feat III), Conv1D(1, 192, None)}  \\ \hline \hline
    \multicolumn{3}{c}{Decoder}                                                       \\ \hline \hline
    \multicolumn{3}{c}{ Fully connected 192 $\rightarrow$ 1 sigmoid }
    \\ \hline
    \end{tabular}
\end{table*}

\begin{table*}[h]
\label{tab:7}
    \centering
    \caption{The network architecture of MBCNN for heart sound segmentation. The example for the illustration of a convolution layer is described as Conv1D (kernel size, output channels, dilation rate, activated function).}
    \begin{tabular}{ccc}                                                            \\ \hline
    \multicolumn{3}{c}{Input: 4000*1 heart sound episode}                                             \\ \hline \hline
    \multicolumn{3}{c}{Encoder}                                                       \\ \hline \hline
    Branch I                  & Branch II                 & Branch III                \\ \hline
    Conv1D (11, 8, 1, 'Relu') & Conv1D (11, 8, 2, 'Relu') & Conv1D (11, 8, 4, 'Relu') \\
    Conv1D (11, 8, 1, 'Relu')  & Conv1D (11, 8, 2, 'Relu')  & Conv1D (11, 8, 4, 'Relu')  \\
    Conv1D (11, 8, 1, 'Relu')  & Conv1D (11, 8, 2, 'Relu')  & Conv1D (11, 8, 4, 'Relu')  \\ \hline
    \multicolumn{3}{c}{Instance Normalization, MaxPool1D(2)}                          \\ \hline
    Conv1D (7, 16, 1, 'Relu')  & Conv1D (7, 16, 4, 'Relu')  & Conv1D (7, 16, 8, 'Relu') \\
    Conv1D (7, 16, 1, 'Relu')  & Conv1D (7, 16, 4, 'Relu')  & Conv1D (7, 16, 8, 'Relu') \\
    Conv1D (7, 16, 1, 'Relu')  & Conv1D (7, 16, 4, 'Relu')  & Conv1D (7, 16, 8, 'Relu') \\ \hline
    \multicolumn{3}{c}{Instance Normalization, MaxPool1D(2)}                          \\ \hline
    \hline
    Conv1D (5, 32, 1, 'Relu')  & Conv1D (5, 32, 8, 'Relu')  & Conv1D (5, 32, 16, 'Relu') \\
    Conv1D (5, 32, 1, 'Relu')  & Conv1D (5, 32, 8, 'Relu')  & Conv1D (5, 32, 16, 'Relu') \\
    Conv1D (5, 32, 1, 'Relu')  & Conv1D (5, 32, 8, 'Relu')  & Conv1D (5, 32, 16, 'Relu') \\ \hline
    \multicolumn{3}{c}{Instance Normalization, MaxPool1D(2)}                          \\ \hline
    \hline
    Conv1D (3, 64, 1, 'Relu')  & Conv1D (3, 64, 16, 'Relu')  & Conv1D (3, 64, 32, 'Relu') \\
    Conv1D (3, 64, 1, 'Relu')  & Conv1D (3, 64, 16, 'Relu')  & Conv1D (3, 64, 32, 'Relu') \\
    Conv1D (3, 64, 1, 'Relu')  & Conv1D (3, 64, 16, 'Relu')  & Conv1D (3, 64, 32, 'Relu') \\ \hline
    \multicolumn{3}{c}{Instance Normalization, MaxPool1D(2)}                          \\ \hline
    Feat I                    & Feat II                   & Feat III                  \\ \hline
    \multicolumn{3}{c}{Concatenate (Feat I, Feat II, Feat III), Conv1D(1, 192, None)}  \\ \hline \hline
    \multicolumn{3}{c}{Decoder}                                                       \\ \hline \hline
    \multicolumn{3}{c}{ Fully connected 192 $\rightarrow$ 4 softmax }                       
    \\ \hline
    \end{tabular}
\end{table*}

For the ablation studies of CCI, we implement MBCNN as the fundamental Encoder.
The network of MBCNN is shown in Tab. VI and Tab. VII for the two tasks, QRS-complex location and heart sound segmentation.
The $\lambda_1$ and $\lambda_2$ in the loss function, Eqn. \ref{eqn:12} are set to $0.1$ and $1$, respectively.
